FoundHand: Large-Scale Domain-Specific Learning for Controllable Hand Image Generation

Despite remarkable progress in image generation models, generating realistic hands remains a persistent challenge due to their complex articulation, varying viewpoints, and frequent occlusions. We present FoundHand, a large-scale domain-specific diffusion model for synthesizing single and dual hand images. To train our model, we introduce FoundHand-10M, a large-scale hand dataset with 2D keypoints and segmentation mask annotations. Our insight is to use 2D hand keypoints as a universal representation that encodes both hand articulation and camera viewpoint. FoundHand learns from image pairs to capture physically plausible hand articulations, natively enables precise control through 2D keypoints, and supports appearance control. Our model exhibits core capabilities that include the ability to repose hands, transfer hand appearance, and even synthesize novel views. This leads to zero-shot capabilities for fixing malformed hands in previously generated images, or synthesizing hand video sequences. We present extensive experiments and evaluations that demonstrate state-of-the-art performance of our method.

==> sec/2_related_work_old.tex <==
\section{Related Works}
\label{sec:related_work}
% Hand reconstruction
% - Geometry Reconstruction 
%     - Statistical model-based reconstruction
%     - Implicit surface-based reconstruction
% - Appearance modeling 

% Diffusion-based 3D generation
% - conditional
% - unconditional

% \section{}
% IIn this section, we review various works related 3D hand reconstruction from RGB images and videos. We also discuss diffusion model-based 3D generation methods as they are related to our work
% \subsection{Hand Reconstruction}
% Hand reconstruction from RGB images is critical to AR/VR applications where realistic hand avatar generation and its articulation are important. We review methods that have proposed solutions to geometry reconstruction only followed by geometry and appearance modelling methods.

% \srinath{Need a section on GANs and diffusion models for image generation.
% Why is there no generative model of hands?}

% \paragraph{Geometry reconstruction} Geometry reconstruction methods have largely relied on statistical models or implicit surfaces for reconstruction. MANO~\cite{mano} is the most widely used statistical model of the hand which provides a parameterization of the pose and shape of the hand. $<$mano parameter estimation methods$>$ $<$direct mesh regression methods$>$ $<$implicit surface estimation methods (HALO)$>$

% \paragraph{Geometry and appearance modelling} LISA, LIVEHAND, HARP
% In this section, we mainly focus on works that obtain realistic images of hands controlled by target poses.

\paragraph{2D Image Generation.}
%
In the past, Generative Adversarial Networks (GANs)~\cite{NIPS2014_5ca3e9b1} have been used extensively to generate images.
Although initial work focused on unconditional generation~\cite{pmlr-v70-arjovsky17a,NIPS2017_892c3b1c,Mescheder2018WhichTM,Miyato2018SpectralNF}, later works have proposed methods for conditional image generation~\cite{Choi2017StarGANUG, Isola2016ImagetoImageTW, Park2019SemanticIS, Kong2019SynthesisAT, Zhang2020CrossDomainCL}.
Closest to our work are methods that generate images of bodies, faces, and hands conditioned on the target pose while preserving the identity of the source image.
\cite{ma2017pose, Chen_2019_CVPR_Workshops,total_gen, Siarohin2017DeformableGF, Wang2019ExampleGuidedSI} use GANs to generate images of human bodies in different poses by conditioning on the source image and target 2D pose or part segmentation map.
\cite{Albahar2021PoseWS} uses correspondence field as condition and utilize StyleGan~\cite{Karras2018ASG} to generate images of a human in target poses. 
\cite{Huang2020LearningIM, Nirkin2019FSGANSA, 3cfaceCAM, towards_3d_face} propose GAN-based methods for human face image generation guided by facial landmarks.
\cite{Deng2020DisentangledAC} uses 3D morphable face model parameters as pose-conditioning and \cite{Ren2021PIRendererCP} uses a latent space for target expression control.
% the  of the target faces.

For hands, \cite{Tang2018GestureGANFH, Hu2021ModelAwareGT} the main focus has been on translating the input hand gesture image to a target gesture image.
% by conditioning on the input and target skeletal poses.
However, in our test, these methods did not generalize well to in-the-wild images.
\cite{sudhakar2024controllingworldsleighthand} transfers the reference hand pose to the target hand mask.
Recently, \cite{Hu2022HandObjectII, Hu2021ModelAwareGT, graspdiffusion, hoidiffusion, genheld, diffh2o} generate images of hand-object grasps by using the target hand and object 3D shapes as conditional inputs.
Unlike these methods, our approach only requires 2D or 3D hand pose readily obtained from off-the-shelf methods~\cite{mediapipe}.
% However, this method requires 3D shape of the hand \srinath{say why our approach is better...}

% \begin{figure}[t]
%     % \renewcommand{\tabcolsep}{2.0pt}
%     \centering \small
%     \begin{tabular}{c}
% \includegraphics[width=0.47\textwidth]{fig/uncondfail.png}\\
% \end{tabular}
% \label{fig:uncondfail}
% \caption{The unconditional models struggle to capture hand articulations.}
% \end{figure}

More recently, diffusion models~\cite{DDPM, improvedDDPM} have increasingly replaced GANs for image synthesis.
Text-guided image diffusion models~\cite{stablediffusion, Saharia2022PhotorealisticTD} powered by large language models~\cite{devlin2018bert,radford2021learning} have been shown to be very effective in generating realistic images.
ControlNet~\cite{controlnet} (and extensions that use 3D structure~\cite{narasimhaswamytext}) provides a framework for fine-tuning diffusion models trained on large-scale data by providing control inputs such as keypoints, segmentation maps, or contours.
% \shreyas{Why does controlnet trained from scratch perform worse than our work?}
However, those conditions lack geometric alignment with the targeted image and hence result in sub-optimal configuration of the fingers and hands. 
% The literature on pose-guided diffusion models for human body, face, or hands is limited to extensions of ControlNet to include 3D structure~\cite{narasimhaswamytext}.
~\cite{exavatar, dreamoving, signllm} generates human video including hands~\cite{human_video_survey}, but those works are limited only to human video or 4D generation, our ours has zero-shot transfer abilities to other tasks.
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\textwidth]{figs/method.pdf}
    \caption{(a) During training, we randomly sample two frames from a video sequence or two different views of a frame as the reference and target frame and encode them using a pretrained VAE as the latent diffusion model. We concatenate the encoded image latent $\mathscr{I}$ with keypoint heatmaps $\mathscr{H}$ and hand mask $\mathscr{M}$ and encode them with a shared-weight embedder to acquire spatially-aligned feature patches before feeding to transformer with 3D self-attention. We don't require target hand mask at test time so we set $\mathscr{M}_{tar}=\emptyset$. $y$ indicates if the two frames are from the same view. (b) For novel view synthesis, we autoregressively sample new views $C_n$ by randomly conditioning the reference frame on one of the previously sampled views or the reference view $\{C_{ref}, C_1, C_2, ..., C_{n-1}\}$ at each denoising step.}
    \label{fig:method}
\end{figure*}
% \paragraph{3D-Model Based Methods} 
% %
% Realistic images of hands in novel poses can also be obtained by rendering textured 3D meshes or neural implicit 3D surfaces that are often learned from multi-view data.
% \cite{Corona2022LISALI} learns an implicit representation of the hand appearance and geometry from a multi-view dataset and can render realistic images of the hand under different poses and shapes. \cite{livehand, manus} learns an implicit texture field with and without MANO~\cite{mano} as the geometry prior and shows that realistic hand avatars can be obtained from a multi-view dataset.
% \cite{harp, ohta} reconstructs a photo-realistic hand avatar using standard explicit representation from a monocular RGB video.
% \cite{html} builds a PCA-based hand appearance model that can be used with the geometry model of MANO.
% \cite{nimble} builds a detailed hand geometry from MRI scans.
% % modeling the bones and muscles, and also uses PCA to obtain the appearance model.
% % Linear models such as PCA have limited expressibility of the detailed hand texture due to their compression into a lower dimensional space.
% Recently, \cite{handiffuser, attentionhand, hand1000} proposed to generate realistic hand images with background, conditioned on text. 
% However, they require 3D hand model as intermediate representation.
% Unlike most 3D-modelling-based methods which require sophisticated capture setups to learn the detailed hand models, our 2D generative method requires only monocular images.
% % and can generate realistic hand images.
% % while still preserving the geometry. 

\paragraph{Datasets.}
%
Numerous datasets have been proposed that contain images of hands~\cite{interhand,simon2017hand,mueller2018ganerated,OccludedHands_ICCV2017,hasson:hal-02429093,zimmermann2019freihand, diva360, oakink2, hograspnet}.
Many focus on a specific scenario such as multi-camera settings, or synthetic hands.
Our goal is to build a model that uses a large amount of hand data.
% but also provides in-the-wild generalization.
We curate a dataset with 2.5M images, 1M from InterHand2.6M~\cite{interhand}, 1M from Ego-4D~\cite{ego4d}, and 500K from FreiHand~\cite{zimmermann2019freihand}, Hanco~\cite{ZimmermannAB21} and HOI4D~\cite{liu2022hoi4d}.
If 2D hand poses are unavailable is available, we automatically extract and crop hand images using Mediapipe~\cite{mediapipe}.
% which has 2.59M images in total, we also automatically extract hands from the EPIC Kitchens~\cite{epickitchen} dataset.
% Together, we gathered \todo{3M} images from these datasets to train our model.

% \paragraph{Applications.}
% %
% Generative image models are increasingly being used for solving inverse problems like correspondence matching~\cite{tang2023dift,hedlin2023unsupervised} and segmentation~\cite{xu2023open}.
% Several works have focused on single-image novel view synthesis of rigid objects~\cite{Liu2023Zero1to3ZO,zero123++,wonder3d} using a diffusion model conditioned on the camera viewpoint and source image.
% Other approaches extend this to 3D reconstruction from a single view~\cite{liu2023one,anciukevivcius2023renderdiffusion,nerdi,syncdreamer,Zhou2022SparseFusionDV}.
% However, all these methods rely some fine-tuning with some form of 3D supervision.
% Text-to-3D shape models~\cite{dreamfusion,wang2023prolificdreamer} have shown that it is possible to reconstruct 3D shape from only a 2D generative model using Score Distillation Sampling (SDS).

% % \cite{Zhou2022SparseFusionDV} learns a view-conditioned diffusion model in the latent space with one or more views as a condition.
% % \cite{wonder3d} uses condition on camera view point, text embedding and domain information to generate images in the novel view.
% % \cite{syncdreamer} proposes a view-conditioned diffusion model that models the joint distribution of the multi-view images.

% To our knowledge, \modelname is the first generative model that is designed exclusively for pose-conditioned generation of hand images.
% When trained on large-scale hand data, our method has the capability to generate realistic and plausible hand images in addition to enabling new applications in novel view synthesis, 3D reconstruction and gesture transfer.
